WKB Method and Quantum Periods beyond Genus One

We extend topological string methods in order to perform WKB approximations for quantum mechanical problems with higher order potentials efficiently. This requires techniques for the evaluation of the relevant quantum periods for Riemann surfaces beyond genus one. The basis of these quantum periods is fixed using the leading behaviour of the classical periods. The full expansion of the quantum periods is obtained using a system of Picard-Fuchs like operators for a sequence of integrals of meromorphic forms of the second kind. Discrete automorphisms of simple higher order potentials allow to view the corresponding higher genus curves as covering of a genus one curve. In this case the quantum periods can be alternatively obtained using the holomorphic anomaly solved in the holomorphic limit within the ring of quasi modular forms of a congruent subgroup of SL$(2,\mathbb{Z})$ as we check for a symmetric sextic potential.

==> highpfops.tex <==
%=======================================================
\section{Higher Order Picard-Fuchs Operators}
\label{sec_highpfops}
%=======================================================

As explained in section \ref{sec_geometry} we can also compute Picard-Fuchs operators which correspond to the higher order WKB periods. For the sextic and quintic oscillator we list here the operators corresponding to order $\hbar^2$ and $\hbar^4$.\\
For the sextic they are
\begin{scriptsize}
\begin{gleichung}
	\mathcal L_\text{PF}^2	&=	\xi  \left(54 \xi ^2-1\right) \left(\num{1782} \xi ^2-65\right)~\partial_\xi^3 + 3 \left(\num{224532} \xi ^4-\num{11124} \xi ^2+65\right)~\partial_\xi^2	\\
			&\qquad+66 \xi  \left(\num{14418} \xi ^2-947\right)~\partial_\xi	+96 \left(\num{1782} \xi ^2-185\right)\\ \phantom{hi} \\
%
	\mathcal L_\text{PF}^4	&=	\xi  \left(54 \xi ^2-1\right) \left(\num{7409920500} \xi ^4-\num{330245820} \xi ^2+\num{9632693}\right)~\partial_\xi^3\\
		&\quad+5 \left(\num{880298555400} \xi ^6-\num{47848497228} \xi ^4+\num{1758643758} \xi ^2-\num{9632693}\right)~\partial_\xi^2\\
		&\qquad+30 \xi  \left(\num{398653722900} \xi ^4-\num{24604325820} \xi ^2+\num{1016813357}\right)~\partial_\xi\\
		&\quad\qquad+960 \left(\num{7409920500} \xi ^4-\num{486072540} \xi ^2+\num{40410853}\right)~.	\\
		\phantom{\mathcal L}
\label{pfsextic6}
\end{gleichung}\noindent
\end{scriptsize}
For the quintic we find
\begin{scriptsize}
\begin{gleichung}\mathcal L_\mathrm{PF}^2 &= 2\left(	 \num{32000000} \xi^3 + \num{193347}	\right)\left(	 \num{25000} \xi^3 - 27	\right)\xi\ \partial_\xi^4 \\
						&\quad	+ 8\left( \num{2600000000000} \xi^6+\num{19118700000} \xi^3-\num{5220369}	\right)\ \partial_\xi^3\\
						&\qquad	+\num{125000}\left(	\num{573440000} \xi ^3+\num{5525577}	\right) \xi ^2\ \partial_\xi^2\\
						&\quad\qquad	+ \num{18000}\left(	\num{3656000000} \xi ^3+\num{49908357} \right) \xi\ \partial_\xi \\
						&\qquad\qquad	+ \num{267995}\left(	\num{32000000} \xi ^3+\num{720657}	\right)\\ \phantom{hi} \\
%
	\mathcal L_\mathrm{PF}^4 =& 2\xi\left(	 \num{25000} \xi ^3-27	\right)\left(	 \num{33013760000000000} \xi ^6+\num{1565984563200000} \xi ^3+\num{6305572607481}	\right)\ \partial_\xi^4 \\
						&\quad	+ 36\left( \num{825344000000000000000} \xi ^9+\num{45674549760000000000} \xi ^6+\num{203138823048300000} \xi ^3\right. \\
				&\hspace{11cm}\left. -\num{56750153467329}	\right)\ \partial_\xi^3\\
						&\qquad	+\num{5000}\left(	\num{31726223360000000000} \xi ^6+\num{2051693233459200000} \xi ^3+\num{11526405450672231}	\right) \xi ^2\ \partial_\xi^2\\
						&\quad\qquad	+ \num{14000}\left(	\num{19890790400000000000} \xi ^6+\num{1504793310105600000} \xi ^3+\num{11080573290031581}\right) \xi\ \partial_\xi \\
						&\qquad\qquad	+ \num{1216215}\left(	\num{99041280000000000} \xi ^6+\num{8399258009600000} \xi ^3+\num{109484562862143}	\right)~.
\label{pfquinticorder4}
\end{gleichung}\noindent
\end{scriptsize}
It is interesting that the higher order Picard-Fuchs operators it seems that new singularities arise because additional factors in front of the highest derivative show up. These are spurious poles since transforming to them we find that no cycle vanishes. Only at roots of the discriminant cycles can vanish as expected from the discussion in section \ref{sec_geometry}. \\
\red{reicht das zu spurious poles?}





